Seshadri Constants and Fujita's Conjecture via Positive Characteristic Methods

In 1988, Fujita conjectured that there is an effective and uniform way to turn an ample line bundle on a smooth projective variety into a globally generated or very ample line bundle. We study Fujita's conjecture using Seshadri constants, which were first introduced by Demailly in 1992 with the hope that they could be used to prove cases of Fujita's conjecture. While examples of Miranda seemed to indicate that Seshadri constants could not be used to prove Fujita's conjecture, we present a new approach to Fujita's conjecture using Seshadri constants and positive characteristic methods. Our technique recovers some known results toward Fujita's conjecture over the complex numbers, without the use of vanishing theorems, and proves new results for complex varieties with singularities. Instead of vanishing theorems, we use positive characteristic techniques related to the Frobenius-Seshadri constants introduced by Musta\c{t}\u{a}-Schwede and the author. As an application of our results, we give a characterization of projective space using Seshadri constants in positive characteristic, which was proved in characteristic zero by Bauer and Szemberg.

==> layout/notation.tex <==
\begingroup
\setlength{\tabcolsep}{3pt}
\begin{longtable}{%
  p{\dimexpr 0.105\linewidth-2\tabcolsep}
  p{\dimexpr 0.395\linewidth-2\tabcolsep}
  p{\dimexpr 0.105\linewidth-2\tabcolsep}
  p{\dimexpr 0.395\linewidth-2\tabcolsep}}
    \toprule
    \endfirsthead
    %
    \toprule
    \multicolumn{4}{l}{(\textsl{\ldots continued from previous page})} \\   
    \endhead
    %
    \multicolumn{4}{l}{(\textsl{continued on next page\ldots})} \\
    \bottomrule
    \endfoot
    %
    \bottomrule
    \endlastfoot
    
    \multicolumn{4}{l}{\textbf{Number systems}}\\
    $\NN$ & natural numbers $\{0,1,\ldots\}$ & $\RR$ & real
    numbers\\
    $\ZZ$ & integers & $\CC$ & complex numbers\\
    $\QQ$ & rational numbers & $\FF_q$ & finite field of order $q$\\
    \midrule
    \multicolumn{4}{l}{\textbf{Commutative algebra}}\\
    $R^\circ$ & \multicolumn{3}{l}{complement of the union of minimal primes}\\
    $N^*_M$ & tight closure\\
    $E_R(M)$ & injective hull of a module $M$\\
    $R^\Gamma$ & the gamma construction\\
    \midrule
    \multicolumn{4}{l}{\textbf{Sheaves}}\\
    $\cO_X$ & structure sheaf & $\omega_X^\bullet$ & dualizing complex\\
    $\cO_X(D)$ & sheaf associated to a divisor & $\omega_X$
    & canonical sheaf\\
    \midrule
    \multicolumn{4}{l}{\textbf{Special algebraic varieties}}\\
    $\PP^n_k$ & $n$-dimensional projective space
\end{longtable}
\endgroup

